Classification of Cell Images Using MPEG-7-influenced Descriptors and Support Vector Machines in Cell Morphology

Counting and classifying blood cells is an important diagnostic tool in medicine. Support Vector Machines are increasingly popular and efficient and could replace artificial neural network systems. Here a method to classify blood cells is proposed using SVM. A set of statistics on images are implemented in C++. The MPEG-7 descriptors Scalable Color Descriptor, Color Structure Descriptor, Color Layout Descriptor and Homogeneous Texture Descriptor are extended in size and combined with textural features corresponding to textural properties perceived visually by humans. From a set of images of human blood cells these statistics are collected. A SVM is implemented and trained to classify the cell images. The cell images come from a CellaVision DM-96 machine which classify cells from images from microscopy. The output images and classification of the CellaVision machine is taken as ground truth, a truth that is 90-95% correct. The problem is divided in two -- the primary and the simplified. The primary problem is to classify the same classes as the CellaVision machine. The simplified problem is to differ between the five most common types of white blood cells. An encouraging result is achieved in both cases -- error rates of 10.8% and 3.1% -- considering that the SVM is misled by the errors in ground truth. Conclusion is that further investigation of performance is worthwhile.

==> fltpoint.tex <==
%%
%% This is file `fltpoint.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% fltpoint.dtx  (with options: `fltmain')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from fltpoint.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file fltpoint.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\edef\atcatcode{\the\catcode`\@}
\catcode`\@=11
\ifx\documentclass\relax
\long\def\@ifnextchar#1#2#3{%
  \let\reserved@d=#1%
  \def\reserved@a{#2}%
  \def\reserved@b{#3}%
  \futurelet\@let@token\@ifnch}
\def\@ifnch{%
  \ifx\@let@token\@sptoken
    \let\reserved@c\@xifnch
  \else
    \ifx\@let@token\reserved@d
      \let\reserved@c\reserved@a
    \else
      \let\reserved@c\reserved@b
    \fi
  \fi
  \reserved@c}
\def\:{\let\@sptoken= } \:
\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@token\@ifnch}
\fi
\def\iloop#1\irepeat{\def\ibody{#1}\iiterate}
\def\iiterate{\ibody\let\inext=\iiterate\else\let\inext=\relax\fi
   \inext}
\def\xloop#1\xrepeat{\def\xbody{#1}\xiterate}
\def\xiterate{\xbody\let\xnext\xiterate\else\let\xnext\relax\fi\xnext}
\let\repeat\fi
\let\irepeat\fi
\let\xrepeat\fi
\newcount\fp@loopcount
\newcount\fp@loopcountii
\newcount\fp@result
\newcount\fp@carryover
\newcount\fp@tempcount
\newcount\fp@tempcountii
\def\fp@setparam#1{\xdef\fp@param{#1}}%
\def\ar@set#1#2#3{\expandafter\edef\csname#1@\number#2\endcsname{%
   \number#3}}
\def\ar@get#1#2{\csname#1@\number#2\endcsname}
\def\ar@setsig#1#2{\expandafter\edef\csname#1@sig\endcsname{#2}}
\def\ar@getsig#1{\csname#1@sig\endcsname}
\def\ar@getul#1{\csname#1@ul\endcsname}
\def\ar@getll#1{\csname#1@ll\endcsname}
\def\ar@setul#1#2{\expandafter\edef\csname#1@ul\endcsname{\number#2}}
\def\ar@setll#1#2{\expandafter\edef\csname#1@ll\endcsname{\number#2}}
\def\fp@settomax#1#2#3{%
   \ifnum#2<#3\relax
      #1=#3\relax
   \else
      #1=#2\relax
   \fi
}
\def\fp@settomin#1#2#3{%
   \ifnum#2<#3\relax
      #1=#2\relax
   \else
      #1=#3\relax
   \fi
}
\def\fp@modulo#1#2{%
   \fp@tempcount=#1\relax
   \fp@tempcountii=#1\relax
   \divide\fp@tempcountii#2\relax
   \multiply\fp@tempcountii#2\relax
   \advance\fp@tempcount-\fp@tempcountii
   \edef\fp@param{\number\fp@tempcount}}
\def\fp@regread#1#2{%
   \fp@regread@raw{#1}{#2}%
   \fp@cleanreg{#1}}
\def\fp@regread@raw#1#2{%
   \fp@tempcount=0
   \edef\fp@arrayname{#1}%
   \ar@setsig{#1}{+}%
   \edef\fp@scratch{#2\fp@decimalsign}%
   \expandafter\fp@readchars\fp@scratch\end
   \ifnum\ar@getul{#1}=-1
      \ar@setul{#1}{0}%
      \ar@set{#1}{0}{0}%
   \fi
   \fp@tempcount=0
   \fp@tempcountii=\ar@getul{#1}\relax
   \iloop
   \ifnum\fp@tempcount<\fp@tempcountii
      \edef\fp@scratch{\ar@get{#1}{\fp@tempcountii}}%
      \ar@set{#1}{\fp@tempcountii}{\ar@get{#1}{\fp@tempcount}}%
      \ar@set{#1}{\fp@tempcount}{\fp@scratch}%
      \advance\fp@tempcount by 1
      \advance\fp@tempcountii by -1
   \irepeat
}% end \fp@regread@raw
\def\fp@readchars#1{%
   \ifx#1\end
      \let\inext=\relax
      \ifnum\fp@tempcount<0
         \advance\fp@tempcount by 1
         \ar@setll{\fp@arrayname}{\fp@tempcount}%
      \else
         \ar@setll{\fp@arrayname}{0}%
      \fi
   \else % \ifx#1\end
      \let\inext=\fp@readchars
      \ifx#1+%
      \else
         \ifx#1-%
            \if\ar@getsig{\fp@arrayname}-%
               \ar@setsig{\fp@arrayname}{+}%
            \else
               \ar@setsig{\fp@arrayname}{-}%
            \fi
         \else
            \if\noexpand#1\fp@decimalsign%
               \ifnum\fp@tempcount>-1
                  \advance\fp@tempcount by -1
                  \ar@setul{\fp@arrayname}{\fp@tempcount}%
                  \fp@tempcount=-1
               \fi
            \else
               \ar@set{\fp@arrayname}{\fp@tempcount}{#1}%
               \ifnum\fp@tempcount<0
                  \advance\fp@tempcount by -1
               \else
                  \advance\fp@tempcount by 1
               \fi
            \fi% end \if\noexpand#1\fp@decimalsign
         \fi% end \ifx#1-
      \fi% end \ifx#1+
   \fi% end \ifx#1\end
   \inext
}% end \fp@readchars
\def\fp@regget#1#2{%
   \if\ar@getsig{#1}-%
      \def#2{-}%
   \else
      \def#2{}%
   \fi
   \fp@tempcount=\ar@getul{#1}\relax
   \iloop
      \ifnum\fp@tempcount=-1
         \edef#2{#2\fp@decimalsign}%
      \fi
      \edef#2{#2\ar@get{#1}{\fp@tempcount}}%
   \ifnum\fp@tempcount>\ar@getll{#1}\relax
      \advance\fp@tempcount by -1
   \irepeat
}% end \def\fp@regget
\def\fp@cleanreg#1{%
   \fp@tempcount=\ar@getul{#1}\relax
   \iloop
   \ifnum\fp@tempcount>0
      \ifnum\ar@get{#1}{\fp@tempcount}=0
         \advance\fp@tempcount by -1
         \ar@setul{#1}{\fp@tempcount}%
      \else
         \fp@tempcount=0
      \fi
   \irepeat
   \fp@tempcount=\ar@getll{#1}\relax
   \iloop
   \ifnum\fp@tempcount<0
      \ifnum\ar@get{#1}{\fp@tempcount}=0
         \advance\fp@tempcount by 1
         \ar@setll{#1}{\fp@tempcount}%
      \else
         \fp@tempcount=0
      \fi
   \irepeat
   \ifnum\ar@getll{#1}=\ar@getul{#1}\relax
      \ifnum\ar@get{#1}{0}=0\relax
         \ar@setsig{#1}{+}%
      \fi
   \fi
}% end \fp@regclean
\def\fp@getdigit#1#2{%
   \ifnum#2<\ar@getll{#1}\relax
      \fp@setparam0%
   \else
      \ifnum#2>\ar@getul{#1}\relax
         \fp@setparam0%
      \else
         \fp@setparam{\ar@get{#1}{#2}}%
      \fi
   \fi
}% end \fp@getdigit
\def\fp@shiftright#1#2{%
   \edef\fp@shiftamount{\number#2}%
   \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{-\fp@shiftamount}%
   \fp@settomin{\fp@tempcountii}{\ar@getll{#1}}{-\fp@shiftamount}%
   \def\fp@shiftnum{}%
   \iloop
      \fp@getdigit{#1}{\fp@tempcount}%
      \edef\fp@shiftnum{\fp@shiftnum\fp@param}%
      \ifnum\fp@tempcount=-\fp@shiftamount\relax
         \edef\fp@shiftnum{\fp@shiftnum\fp@decimalsign}%
      \fi
   \ifnum\fp@tempcount>\fp@tempcountii
      \advance\fp@tempcount by -1
   \irepeat
   \fp@regread{#1}{\fp@shiftnum}%
}% end \fp@shiftright
\def\fp@firstnonzero#1{%
   \fp@regcomp{#1}{@0}%
   \if\fp@param=%
      \fp@setparam0%
   \else
      \fp@tempcount=\ar@getul{#1}\relax%
      \fp@tempcountii=\ar@getll{#1}\relax%
      \iloop
         \ifnum\ar@get{#1}{\fp@tempcount}>0
            \fp@setparam{\number\fp@tempcount}%
            \fp@tempcount=\fp@tempcountii
         \fi
      \ifnum\fp@tempcount>\fp@tempcountii
         \advance\fp@tempcount by -1
      \irepeat
   \fi
}% end \fp@firstnonzero
\def\fp@regcomp#1#2{%
   {%
      \if\ar@getsig{#1}-%
         \if\ar@getsig{#2}-%
            \fp@regcomp@main{#1}{#2}<>%
         \else
            \fp@setparam{<}%
         \fi
      \else
         \if\ar@getsig{#2}-%
            \fp@setparam{>}%
         \else
            \fp@regcomp@main{#1}{#2}><%
         \fi
      \fi
   }%
}
\def\fp@regcomp@main#1#2#3#4{%
   \fp@settomax{\fp@loopcount}{\ar@getul{#1}}{\ar@getul{#2}}%
   \fp@settomin{\fp@loopcountii}{\ar@getll{#1}}{\ar@getll{#2}}%
   \loop
      \fp@getdigit{#1}{\fp@loopcount}%
      \fp@tempcount=\fp@param\relax
      \fp@getdigit{#2}{\fp@loopcount}%
      \fp@tempcountii=\fp@param\relax
      \ifnum\fp@tempcount<\fp@tempcountii
         \fp@setparam{#4}%
         \fp@loopcount=\fp@loopcountii
      \else
         \ifnum\fp@tempcount>\fp@tempcountii
            \fp@setparam{#3}%
            \fp@loopcount=\fp@loopcountii
         \else
            \ifnum\fp@loopcount=\fp@loopcountii
               \fp@setparam{=}%
            \fi
         \fi
      \fi
   \ifnum\fp@loopcount>\fp@loopcountii
      \advance\fp@loopcount by -1
   \repeat
}% end \fp@regcomp@main
\def\fp@regabs#1{%
   \ar@setsig{#1}{+}%
}
\def\fp@regneg#1{%
   \if\ar@getsig{#1}-%
      \ar@setsig{#1}{+}%
   \else
      \fp@regcomp{#1}{@0}%
      \if\fp@param=%
      \else
         \ar@setsig{#1}{-}%
      \fi
   \fi
}
\def\fp@reground#1#2{%
   \ifnum#2>\ar@getll{#1}\relax
      {%
         \fp@tempcount=#2\relax
         \advance\fp@tempcount by -1
         \fp@getdigit{#1}{\fp@tempcount}%
         \ifnum\fp@param>4
            \fp@regcopy{fp@temp}{@1}%
            \fp@shiftright{fp@temp}{#2}%
            \fp@regcomp{#1}{@0}%
            \if\fp@param<%
               \fp@regneg{fp@temp}%
            \fi
            \fp@regadd{#1}{fp@temp}%
         \fi
         \ifnum#2>0
            \fp@loopcount=#2\relax
            \iloop
               \ifnum\fp@loopcount>0
                  \advance\fp@loopcount by -1
                  \ar@set{#1}{\fp@loopcount}{0}%
            \irepeat
            \ar@setll{#1}{0}%
         \else
            \ar@setll{#1}{#2}%
         \fi
         \fp@regget{#1}{\fp@scratch}%
         \fp@setparam\fp@scratch
      }%
      \fp@regread{#1}{\fp@param}%
   \fi
} % end \fp@reground
\def\fp@regcopy#1#2{%
   \fp@regget{#2}{\fp@scratch}%
   \fp@regread{#1}{\fp@scratch}%
}
\def\fp@regadd#1#2{%
   {%
      \if\ar@getsig{#1}\ar@getsig{#2}%
         \fp@settomin{\fp@loopcount}{\ar@getll{#1}}{\ar@getll{#2}}%
         \edef\fp@add@start{\number\fp@loopcount}%
         \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{\ar@getul{#2}}%
         \edef\fp@add@finish{\number\fp@tempcount}%
         \fp@carryover=0
         \loop
            \fp@getdigit{#1}{\fp@loopcount}%
            \fp@result=\fp@param\relax
            \fp@getdigit{#2}{\fp@loopcount}%
            \advance\fp@result by \fp@param\relax
            \advance\fp@result by \fp@carryover
            \ifnum\fp@result>9
               \fp@carryover=1
               \advance\fp@result by -10
            \else
               \fp@carryover=0
            \fi
            \ar@set{#1}{\fp@loopcount}{\fp@result}%
         \ifnum\fp@loopcount<\fp@add@finish\relax
            \advance\fp@loopcount by 1
         \repeat
         \ifnum\fp@carryover>0
            \advance\fp@loopcount by 1
            \ar@set{#1}{\fp@loopcount}{\fp@carryover}%
         \fi
         \ar@setll{#1}{\fp@add@start}%
         \ar@setul{#1}{\fp@loopcount}%
         \fp@regget{#1}{\fp@scratch}%
         \fp@setparam\fp@scratch
      \else % \if sign
         \fp@regcopy{fp@tempi}{#1}%
         \fp@regcopy{fp@tempii}{#2}%
         \fp@regabs{fp@tempi}%
         \fp@regabs{fp@tempii}%
         \fp@regcomp{fp@tempi}{fp@tempii}%
         \if\fp@param>%
            \fp@regadd@sub{#1}{fp@tempi}{fp@tempii}%
         \else
            \fp@regadd@sub{#2}{fp@tempii}{fp@tempi}%
         \fi
      \fi % end \if sign
   }%
   \fp@regread{#1}{\fp@param}%
}% end \fp@regadd
\def\fp@regadd@sub#1#2#3{%
   \fp@regsub@restricted{#2}{#3}%
   \fp@regcomp{#1}{@0}%
   \if\fp@param<%
      \fp@regneg{#2}%
   \fi
   \fp@regget{#2}{\fp@scratch}%
   \fp@setparam\fp@scratch
}% end \fp@regadd@sub
\def\fp@regsub@restricted#1#2{%
   {%
      \fp@settomin{\fp@loopcount}{\ar@getll{#1}}{\ar@getll{#2}}%
      \edef\fp@lowermin{\number\fp@loopcount}%
      \fp@settomax{\fp@tempcount}{\ar@getul{#1}}{\ar@getul{#2}}%
      \edef\fp@uppermin{\number\fp@tempcount}%
      \fp@carryover=0
      \loop
         \fp@getdigit{#1}{\fp@loopcount}%
         \fp@result=\fp@param\relax
         \fp@getdigit{#2}{\fp@loopcount}%
         \advance\fp@result by -\fp@param\relax
         \advance\fp@result by \fp@carryover
         \ifnum\fp@result<0
            \fp@carryover=-1
            \advance\fp@result by 10
         \else
            \fp@carryover=0
         \fi
         \ar@set{#1}{\fp@loopcount}{\fp@result}%
      \ifnum\fp@loopcount<\fp@uppermin\relax
         \advance\fp@loopcount by 1
      \repeat
      \ifnum\fp@carryover=-1
         \advance\fp@loopcount by 1
         \ar@set{#1}{\fp@loopcount}{-1}%
      \fi
      \ar@setll{#1}{\fp@lowermin}%
      \ar@setul{#1}{\fp@loopcount}%
   \fp@regget{#1}{\fp@scratch}%
   \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}% end \fp@regsub@restricted
\def\fp@regsub#1#2{%
   {%
      \fp@regneg{#2}%
      \fp@regadd{#1}{#2}%
      \fp@regget{#1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}
\def\fp@regmul#1#2{%
   {%
      \fp@regcopy{fp@temp1}{@0}%
      \fp@loopcountii=\ar@getll{#2}\relax
      \xloop
         \fp@loopcount=\ar@getll{#1}\relax
         \fp@carryover=0
         \def\fp@newnum{}%
         \loop
            \fp@result=\ar@get{#2}{\fp@loopcountii}\relax
            \multiply\fp@result by \ar@get{#1}{\fp@loopcount}\relax
            \advance\fp@result by \fp@carryover
            \ifnum\fp@result>9
               \fp@carryover=\fp@result
               \divide\fp@carryover by 10
               \fp@tempcount=\fp@carryover
               \multiply\fp@tempcount by 10
               \advance\fp@result by -\fp@tempcount
            \else
               \fp@carryover=0
            \fi
            \edef\fp@newnum{\number\fp@result\fp@newnum}%
         \ifnum\fp@loopcount<\ar@getul{#1}\relax
            \advance\fp@loopcount by 1
         \repeat
         \edef\fp@newnum{\number\fp@carryover\fp@newnum}%
         \fp@regread{fp@temp2}{\fp@newnum}%
         \fp@tempcount=\fp@loopcountii
         \advance\fp@tempcount by -\number\ar@getll{#2}\relax
         \fp@shiftright{fp@temp2}{\fp@tempcount}%
         \fp@regadd{fp@temp1}{fp@temp2}%
      \ifnum\fp@loopcountii<\ar@getul{#2}\relax
         \advance\fp@loopcountii by 1
      \xrepeat
      \fp@tempcount=\ar@getll{#1}\relax
      \advance\fp@tempcount by \ar@getll{#2}\relax
      \fp@shiftright{fp@temp1}{\fp@tempcount}%
      \if\ar@getsig{#1}\ar@getsig{#2}%
      \else
         \fp@regneg{fp@temp1}%
      \fi
   \fp@regget{fp@temp1}{\fp@scratch}%
   \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
} % end \fp@regmul
\def\fp@regdiv#1#2{%
   {%
      \fp@regcopy{fp@temp1}{#1}%
      \fp@regcopy{fp@temp2}{#2}%
      \fp@regabs{fp@temp1}%
      \fp@regabs{fp@temp2}%
      \fp@firstnonzero{fp@temp1}%
      \fp@loopcountii=\fp@param\relax
      \fp@firstnonzero{fp@temp2}%
      \advance\fp@loopcountii by -\fp@param\relax
      \fp@shiftright{fp@temp2}{\fp@loopcountii}%
      \def\fp@divnum{}%
      \ifnum\fp@loopcountii<0
         \fp@tempcount=\fp@loopcountii
         \loop
         \ifnum\fp@tempcount<-1
            \edef\fp@divnum{0\fp@divnum}%
            \advance\fp@tempcount by 1
         \repeat
         \edef\fp@divnum{\fp@decimalsign\fp@divnum}%
      \fi
      \xloop
      \fp@tempcount=\fp@loopcountii
      \advance\fp@tempcount by 1
      \ifnum\fp@tempcount>-\fp@accuracy\relax
         \fp@loopcount=0
         \loop
            \fp@regcomp{fp@temp2}{fp@temp1}%
            \if\fp@param=%
               \def\fp@accuracy{0}%
               \gdef\fp@param{<}%
            \fi
         \if\fp@param<%
            \fp@regsub@restricted{fp@temp1}{fp@temp2}%
            \advance\fp@loopcount by 1
         \repeat
         \ifnum\fp@loopcountii=-1
            \edef\fp@divnum{\fp@divnum\fp@decimalsign}%
         \fi
         \edef\fp@divnum{\fp@divnum\number\fp@loopcount}%
         \fp@shiftright{fp@temp2}{-1}%
         \advance\fp@loopcountii by -1
      \xrepeat
      \if\ar@getsig{#1}\ar@getsig{#2}%
         \fp@regread{fp@temp1}{\fp@divnum}%
      \else
         \fp@regread{fp@temp1}{-\fp@divnum}%
      \fi
      \fp@regget{fp@temp1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \fp@regread{#1}{\fp@param}%
}
\def\fp@call@bin#1#2#3#4{%
   {%
      \fp@regread{fp@user1}{#2}%
      \fp@regread{fp@user2}{#3}%
      \csname fp@reg#4\endcsname{fp@user1}{fp@user2}%
      \fp@regget{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpAdd#1#2#3{\fp@call@bin{#1}{#2}{#3}{add}}
\def\fpSub#1#2#3{\fp@call@bin{#1}{#2}{#3}{sub}}
\def\fpMul#1#2#3{\fp@call@bin{#1}{#2}{#3}{mul}}
\def\fpDiv#1#2#3{\fp@call@bin{#1}{#2}{#3}{div}}
\def\fp@call@un#1#2#3{%
   {%
      \fp@regread{fp@user1}{#2}%
      \csname fp@reg#3\endcsname{fp@user1}%
      \fp@regget{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpAbs#1#2{\fp@call@un{#1}{#2}{abs}}
\def\fpNeg#1#2{\fp@call@un{#1}{#2}{neg}}
\def\fpRound#1#2#3{%
   {%
      \fpRegSet{fp@user1}{#2}%
      \fpRegRound{fp@user1}{#3}%
      \fpRegGet{fp@user1}{\fp@scratch}%
      \fp@setparam\fp@scratch
   }%
   \edef#1{\fp@param}%
}
\def\fpRegSet#1#2{\fp@regread{#1}{#2}}
\def\fpRegGet#1#2{\fp@regget{#1}{#2}}
\def\fpRegAdd#1#2{\fp@regadd{#1}{#2}}
\def\fpRegSub#1#2{\fp@regsub{#1}{#2}}
\def\fpRegMul#1#2{\fp@regmul{#1}{#2}}
\def\fpRegDiv#1#2{\fp@regdiv{#1}{#2}}
\def\fpRegAbs#1{\fp@regabs{#1}}
\def\fpRegNeg#1{\fp@regneg{#1}}
\def\fpRegCopy#1#2{\fp@regcopy{#1}{#2}}
\def\fpRegRound#1#2{\fp@reground{#1}{#2}}
\def\fpAccuracy#1{\edef\fp@accuracy{#1}}
\fpAccuracy{5}
\def\fpDecimalSign#1{\edef\fp@decimalsign{#1}}
\fpDecimalSign{,}
\def\fpThousandSep#1{\edef\fp@thousandsep{#1}}
\fpThousandSep{}
\fp@regread{@0}{0}
\fp@regread{@1}{1}
\catcode`\@=\atcatcode\relax
\endinput
%%
%% End of file `fltpoint.tex'.

